Mosaic Zonotope Shadow Matching for Risk-Aware Autonomous Localization in Harsh Urban Environments

Risk-aware urban localization with the Global Navigation Satellite System (GNSS) remains an unsolved problem with frequent misdetection of the user's street or side of the street. Significant advances in 3D map-aided GNSS use grid-based GNSS shadow matching alongside AI-driven line-of-sight (LOS) classifiers and server-based processing to improve localization accuracy, especially in the cross-street direction. Our prior work introduces a new paradigm for shadow matching that proposes set-valued localization with computationally efficient zonotope set representations. While existing literature improved accuracy and efficiency, the current state of shadow matching theory does not address the needs of risk-aware autonomous systems. We extend our prior work to propose Mosaic Zonotope Shadow Matching (MZSM) that employs a classifier-agnostic polytope mosaic architecture to provide risk-awareness and certifiable guarantees on urban positioning. We formulate a recursively expanding binary tree that refines an initial location estimate with set operations into smaller polytopes. Together, the smaller polytopes form a mosaic. We weight the tree branches with the probability that the user is in line of sight of the satellite and expand the tree with each new satellite observation. Our method yields an exact shadow matching distribution from which we guarantee uncertainty bounds on the user localization. We perform high-fidelity simulations using a 3D building map of San Francisco to validate our algorithm's risk-aware improvements. We demonstrate that MZSM provides certifiable guarantees across varied data-driven LOS classifier accuracies and yields a more precise understanding of the uncertainty over existing methods. We validate that our tree-based construction is efficient and tractable, computing a mosaic from 14 satellites in 0.63 seconds and growing quadratically in the satellite number.

==> sections/abstract.tex <==
\begin{abstract}
% This template helps you to create a properly formatted \LaTeX\ manuscript.

% Risk-aware urban localization remains an unsolved problem with frequent misdetection of the user's side of the street or even the city block. 
Risk-aware urban localization with the Global Navigation Satellite System (GNSS) remains an unsolved problem with frequent misdetection of the user's street or side of the street.
Without risk-aware localization, autonomous AI agents do not have the state uncertainty information necessary for decision-making.
% Significant advances in 3D map-aided GNSS localization have led to the multi-pronged Intelligent Urban Positioning system that uses shadow matching as a core component to improve cross-street accuracy. 
% Other works have introduced machine learning-based classifiers into shadow matching to improve GNSS satellite line-of-sight detection. 
% However, the core shadow matching algorithm cannot adapt to real-time environment changes, does not provide a method to connect information across satellites, and has difficulties quantifying the uncertainty. 
% The core shadow matching analysis further requires a system designer to incorporate a specific classifier to test the end-to-end process. 
% With the vast space of possible classifiers, one cannot test all classifiers with shadow matching. 
Significant advances in 3D map-aided GNSS use grid-based GNSS shadow matching alongside AI-driven line-of-sight~(LOS) classifiers and server-based processing to improve localization accuracy, especially in the cross-street direction.
% To avoid trade-off between accuracy and compute cost caused by grid-based discretization, In 
% On the other hand, our prior work on set-based shadow matching leverages an efficient set representation, namely zonotope, to compute GNSS shadows that are later sequentially processed to compute an exact set-based receiver position. 
Our prior work introduces a new paradigm for shadow matching that proposes set-valued localization with computationally efficient zonotope set representations.
% is computed. % leveragintsequentially refine the based on a binary LOS/NLOS classifier to compute the final set-based receiver position. 
% , we leverage set representation propose Zonotope Shadow Matching (ZSM) for set-valued 3-D map-aided GNSS localization.
% ZSM represents buildings and GNSS shadows using constrained zonotopes, a type of convex polytope that can propagate set-valued estimates using fast vector concatenation operations.
% Starting from a coarse set-valued position, ZSM refines the estimate depending on the receiver being inside or outside each shadow as judged by received carrier-to-noise density. 
While existing literature improved accuracy and efficiency, the current state of shadow matching theory does not address the needs of risk-aware autonomous systems.
% Therefore, we propose Mosaic Zonotope Shadow Matching, which is the first risk-aware theoretical framework for shadow matching where we can provide classifier-agnostic formal guarantees on the shadow matching uncertainty bounds.
We extend our prior work to propose Mosaic Zonotope Shadow Matching~(MZSM) that employs a classifier-agnostic polytope mosaic architecture to provide risk-awareness and certifiable guarantees on urban positioning.
% We demonstrate that state-of-the-art Gaussian or grid-based approximations are unsuitable for risk-aware shadow matching. 
% To design a classifier-agnostic mosaic, w
We formulate a recursively expanding binary tree that % performs set operations to bifurcates %the area of interest 
% bifurcates a coarse initial estimate
refines an initial location estimate with set operations into smaller polytopes. Together, the smaller polytopes form a mosaic.
% into smaller polytopes with set operations. % at each tree level, and 
% Thereafter, 
We weight the tree branches with the probability that the user is in line of sight of the satellite and expand the tree with each new satellite observation.
% LOS satellite classifier. % at each tree level. %in parallel, percolate the LOS/NLOS classifier probabilities through different tree levels. 
% Our method computes an exact shadow matching distribution, which is later used to compute a confidence collection of smaller polytopes that collectively satisfy a user confidence level. 
Our method yields an exact shadow matching distribution from which we compute a confidence collection of smaller polytopes that guarantees uncertainty bounds on the user localization within specified user confidence.
% bifurcates each tree node into LOS and NLOS branches comprises multiple polytopes with an associated probability  
% To formulate a classifier-agnostic polytope mosaic that comprises , our method models a recursive tree expansion that bifurcates each tree node set operations to compute the exact shadow matching distribution and a tree-based structure to ensure computational efficiency. 
% We provide a tractable and precise understanding of the shadow matching uncertainty in real-time across classifiers and user confidence levels.
We perform high-fidelity simulations using a 3D building map of San Francisco to validate our algorithm's risk-aware improvements as compared to grid-based shadow matching and Gaussian uncertainty models. 
% We demonstrate that current Gaussian uncertainty models incur a high integral error of 0.5, unsuitable for risk-aware localization, whereas our set-based method incurs no error since it computes the exact error model.
% We show that current grid-based methods for shadow matching match the exact set-based methods  for typical classifiers to 75\% in the best case but can be as low as 40\%.
% Grid-based methods can converge to set-based methods for highly refined grids, though such high grid resolutions are too computationally expensive.  
% In particular, we compare against the state-of-the-art GMMs, and conventional grid-based shadow matching to demonstrate our algorithm's improved risk-awareness while ensuring compute efficiency.
We demonstrate that MZSM provides certifiable guarantees across varied data-driven LOS classifier accuracies and yields a more precise understanding of the uncertainty over existing methods. 
Additionally, we validate that our tree-based construction is efficient and tractable, computing a mosaic from 14 satellites in 0.63 seconds and growing quadratically in the satellite number. 
With our analyses, we focus on how system designers can facilitate AI decision-making in urban settings with our risk-aware framework for urban GNSS localization.
% Our tree-based method computes the mosaic of 14 satellites in 0.63 seconds and grows quadratically with satellite number, which enables real-time localization 

% and can compute and validate the sensitivity of our algorithm's performance across LOS/NLOS classifier accuracy and desired user confidence levels. 
% Something about 0.63 seconds.
\end{abstract}

\begin{keyword}
GNSS, Shadow Matching, Set-based, Risk-Aware Localization
%\texttt{elsarticle.cls}\sep \LaTeX\sep Elsevier \sep template
%\MSC[2010] 00-01\sep  99-00
\end{keyword}
